Improving GAN Training via Binarized Representation Entropy (BRE) Regularization

We propose a novel regularizer to improve the training of Generative Adversarial Networks (GANs). The motivation is that when the discriminator D spreads out its model capacity in the right way, the learning signals given to the generator G are more informative and diverse. These in turn help G to explore better and discover the real data manifold while avoiding large unstable jumps due to the erroneous extrapolation made by D. Our regularizer guides the rectifier discriminator D to better allocate its model capacity, by encouraging the binary activation patterns on selected internal layers of D to have a high joint entropy. Experimental results on both synthetic data and real datasets demonstrate improvements in stability and convergence speed of the GAN training, as well as higher sample quality. The approach also leads to higher classification accuracies in semi-supervised learning.

==> related.tex <==
\section{Related}

 
Model capacity in generative adversarial networks (GANs) has been previously explored \cite{arora2017generalization}. 
While they show discriminator $D$ with finite number of parameters cannot detect insufficient diversity in generator $G$'s samples,
the question on \textit{where} and \textit{how} $D$ can utilize its limited capacity effectively is left unanswered. 
In this direction,
our work can be thought of as a method to direct $D$'s finite parameter resources on generated data as well as interpolation between real and generated data. 
This is ``where'' capacity is addressed. 
Morever,
not only should $D$ do well on its classification task, 
but it also needs to tell apart each generated or interpolated sample in \textit{distinct} ways. 
This is ``how'' capacity is used. 
Both are important for GANs, 
because $D$'s role is to learn all features from real data and pass them to $G$ via $\nabla_{x}D(x)$, 
which also distinguishes $D$'s role from regular supervised learning tasks where irrelevant features for the labels can be forgotten. 
However,
the number of parameters for neural nets is a very weak notion for model capacity. 
A finer notion for measuring capacity, 
particularly suited for rectifier nets, 
is activation pattern \cite{raghu2016expressive}. 
In their work,
it is shown that the activation patterns is upper bounded by depth and  
widths. 
Under GANs' finite capacity constraint,
it is thus important to allocate the activation patterns onto interpolated and generated data and not waste the capacity on places where there is no data. 
% More precisely, 
% our regularizer encourages diversities in $D$'s activation pattern \cite{raghu2016expressive} 
% % or more directly its gradient with respect to input,
% % $\nabla_{x}D(x)$,
% on each real or generated data point. 
% % In the former case,
Since activation pattern corresponds to number of piecewise linear regions $D$ cuts into \cite{montufar2014number}, 
each piecewise linear region should contain as few data points as possible. 
As data points $x$ lie in different regions, 
$\nabla_{x}D(x)$ are likely to be diverse. 
$G$ in turn can receive diverse learning signals from $\nabla_{x}D(x)$. 
It is in this sense that we encourage model capacity usage of $D$. 
Henceforth,
we use activation pattern
% or input gradient, $\nabla_{x}D(x)$, 
as a measure on where and how $D$ uses its model capacity. See figure \ref{fig:capacity_regeme} for a pictorial illustration.  
% Note this is a finer notion of model capacity than number of paramters. 





==> theory.tex <==
\input{complexity_overview}
\input{R_sbre}


%% \todoy[inline]{talk about the following when talking about resnet}
%% Since our goal is to have diverse representation of data, so that generator can receive diverse training signals, it might be tempting to just regularize the input-gradient of \D. 
%% Let $\nabla_x L(D(\vc{x}))$ be the gradient of discriminator loss with respect to input, and let $\vc{v}_{k} = \softsign{\nabla_x L(D(\vc{x}_k))}$ be the soft sign vector of gradient on $k$-th data point, the transport direction entropy regularizer is defined as:
%% \begin{equation}
%%   R_{input} = \sum_{k \neq j}  \max(0, |\vc{v}_{k}^{\T}\vc{v}_{j}| - \eta)
%% \end{equation}


